A Simple-but-effective Baseline for Training-free Class-Agnostic Counting

Class-Agnostic Counting (CAC) seeks to accurately count objects in a given image with only a few reference examples. While previous methods achieving this relied on additional training, recent efforts have shown that it's possible to accomplish this without training by utilizing pre-existing foundation models, particularly the Segment Anything Model (SAM), for counting via instance-level segmentation. Although promising, current training-free methods still lag behind their training-based counterparts in terms of performance. In this research, we present a straightforward training-free solution that effectively bridges this performance gap, serving as a strong baseline. The primary contribution of our work lies in the discovery of four key technologies that can enhance performance. Specifically, we suggest employing a superpixel algorithm to generate more precise initial point prompts, utilizing an image encoder with richer semantic knowledge to replace the SAM encoder for representing candidate objects, and adopting a multiscale mechanism and a transductive prototype scheme to update the representation of reference examples. By combining these four technologies, our approach achieves significant improvements over existing training-free methods and delivers performance on par with training-based ones.

==> figures/fig_bubble.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/bubble2.pdf}  
\caption{}
\label{fig:bubble}
\end{figure}

==> figures/rebuttal_ours_vs_pseco.tex <==
\begin{figure}[t]
\vspace{-0.5cm}
\centering
% \includegraphics[width=0.48\linewidth]{images/7611_ous.jpg}  
% \includegraphics[width=0.48\linewidth]{images/7611.jpg}  
\includegraphics[width=0.6\linewidth]{images/pdfresizer.com-pdf-crop.pdf}
\vspace{-0.4cm}
\caption{FSC-147 example results. Zoom in for detail.}
\label{fig:vsPseCo}
\vspace{-0.7cm}
\end{figure}

==> tables/tab_component_carpk.tex <==
\begin{table}[]
\centering
\resizebox{0.75\columnwidth}{!}{

\begin{tabular}{cccc|cc}
\toprule
\multicolumn{3}{c}{Components}  & \multicolumn{2}{c}{CARPK}    \\ 
\cline{1-4} \cline{5-6} 
SP  & DINOv2 & TPU & MAE $\downarrow$ & RMSE $\downarrow$ \\ 
\hline
-               &-            &-                         & 14.27 & 16.61 \\
\checkmark      & -           &  -                    & 19.63 & 21.90  \\
-               & \checkmark  &  -                    & \hm{6.06} & \hm{8.51}  \\
\checkmark      & \checkmark  &   -                   & 4.60 & 6.64  \\
\checkmark      & \checkmark  &\checkmark            & 4.39 & 5.70 \\          
\bottomrule
\end{tabular}}
\caption{Performance with different components on CARPK. SP: superpixel, TPU: transductive prototype updating.}
\label{tab:aba_carpk} 
\end{table}

==> tables/text.tex <==
\begin{table}[h]
\centering
\resizebox{0.95\columnwidth}{!}{
\begin{tabular}{@{}lccccccccccc@{}}
\toprule
&\multirow{2}{*}{\textbf{Training-free}} & \multicolumn{2}{c}{\textbf{FSC-147}}\\
\cmidrule(lr){3-4}
& & \textbf{MAE} $\downarrow$ &
\textbf{RMSE} $\downarrow$ \\
\hline
% Xu \etal \cite{xu2023zero} &Yes&\underline{22.09} &\underline{115.17} &\underline{0.34}&\underline{3.74}\\
SAM Baseline~\cite{shi2023training} &Yes&42.48 &137.50\\
TFOC~\cite{shi2023training} (vanilla) &Yes&32.86 &142.89 \\
TFOC~\cite{shi2023training} &Yes&24.79 &137.15\\

% \rowcolor{Gray}
\textbf{Ours} &Yes&\textbf{14.88} &\textbf{56.91} \\

\bottomrule
\end{tabular}}
\caption{Effect of our approach with text prompt on FSC-147.
}
\label{tab:text-prompt}
\end{table}
